Towards Motion Forecasting with Real-World Perception Inputs: Are End-to-End Approaches Competitive?

Motion forecasting is crucial in enabling autonomous vehicles to anticipate the future trajectories of surrounding agents. To do so, it requires solving mapping, detection, tracking, and then forecasting problems, in a multi-step pipeline. In this complex system, advances in conventional forecasting methods have been made using curated data, i.e., with the assumption of perfect maps, detection, and tracking. This paradigm, however, ignores any errors from upstream modules. Meanwhile, an emerging end-to-end paradigm, that tightly integrates the perception and forecasting architectures into joint training, promises to solve this issue. However, the evaluation protocols between the two methods were so far incompatible and their comparison was not possible. In fact, conventional forecasting methods are usually not trained nor tested in real-world pipelines (e.g., with upstream detection, tracking, and mapping modules). In this work, we aim to bring forecasting models closer to the real-world deployment. First, we propose a unified evaluation pipeline for forecasting methods with real-world perception inputs, allowing us to compare conventional and end-to-end methods for the first time. Second, our in-depth study uncovers a substantial performance gap when transitioning from curated to perception-based data. In particular, we show that this gap (1) stems not only from differences in precision but also from the nature of imperfect inputs provided by perception modules, and that (2) is not trivially reduced by simply finetuning on perception outputs. Based on extensive experiments, we provide recommendations for critical areas that require improvement and guidance towards more robust motion forecasting in the real world. The evaluation library for benchmarking models under standardized and practical conditions is provided: \url{https://github.com/valeoai/MFEval}.

==> tabs/agent_neighbor_noise.tex <==
\begin{table}[t]
\centering

    \caption{Performance of LaPred \cite{yuan2021agentformer} given perturbations in agent-of-interest's or neighbors' trajectories.}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}l c c c c@{}}
    \toprule
    Setting & mAP${_f}$  $\uparrow$ & minADE $\downarrow$  & minFDE $\downarrow$  & MR $\downarrow$ \\

     \midrule  
      Ground truth                             &0.760	& 1.237	& 2.344	& 0.118   \\  
      Agent Loc.Error                           &0.176	& 4.991	& 6.450	& 0.520 \\
      Neighbor Loc.Error                       &0.744	     & 1.291	& 2.474	& 0.125 \\ 
    \bottomrule
    \end{tabular}
    }
  \label{tab:agent_nei_noise}
\end{table}


==> tabs/map_semantic_imperfections.tex <==
\begin{table*}[h]
\centering
    \caption{\yihongh{Drop of performance when removing classes of map elements from the GT map.}}
    
    \resizebox{0.9\linewidth}{!}{
    \begin{tabular}{l l c c c c}
    \toprule
     & & mAP${_f}$  $\uparrow$ & minADE $\downarrow$  & minFDE $\downarrow$  & MR $\downarrow$ \\

     \midrule  
     \parbox[t]{3mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{AgentF.}}} & with GT \eloih{rasterized} HD map                                              &0.388	&1.851	&3.875	&0.315  \\  
       & \hspace{0.5cm} without road polygons                                      &\textbf{-0.092}	&\textbf{+0.171}	&\textbf{+0.453}	&\textbf{+0.072}\\ 
       & \hspace{0.5cm} without road divider                                        &-0.001&	+0.007	&+0.018	&+0.002 \\  
       & \hspace{0.5cm} without lane divider                                      &-0.001	&+0.009	&+0.034	&+0.007 \\  
     \midrule  
     \parbox[t]{3mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{LaPred}}} & with GT \eloih{vectorized} HD map                                              & {0.760}	&{1.237}	&{2.344}	&{0.118} \\  
     & \hspace{0.5cm} without lane                                      &\textbf{-0.149}	&\textbf{+0.272}	&\textbf{+0.664}	&\textbf{+0.093}\\ 
     & \hspace{0.5cm} without lane connector                                      &-0.092	&+0.162	&+0.390	&+0.044\\ 
    \bottomrule
    \end{tabular}
    }
  \label{tab:semantic_map_imperfections}
  \vspace{+5mm}
\end{table*}


==> tabs/real_world_inputs_per_class_w_lapred.tex <==
\begin{table*}[ht]
\centering

\tabcolsep=0.11cm
    \caption{\yihongh{Detailed forecasting results using AgentFormer \cite{yuan2021agentformer} and LaPred \cite{kim2021lapred} with real-world perception inputs.}}
    \vspace{-2mm}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c l| c c c c c | c c c c | c c c c}
    \toprule
     & & \multicolumn{5}{c|}{Tracking metrics} & \multicolumn{8}{c}{Forecasting metrics} \\
    \midrule 
      & & & & & & & \multicolumn{4}{c}{AgentFormer \cite{yuan2021agentformer}} & \multicolumn{4}{c}{LaPred \cite{kim2021lapred}} \\
    \midrule
     & Method & MOTA $\uparrow$ & MOTP $\downarrow$ & FP $\downarrow$ & FN $\downarrow$ & IDS $\downarrow$  & AP$_f$ $\uparrow$  & minADE $\downarrow$ & minFDE$\downarrow$ &  MR $\downarrow$ & AP$_f$ $\uparrow$  & minADE $\downarrow$ & minFDE$\downarrow$ &  MR $\downarrow$\\ [0.5ex]
     \midrule
     \parbox[t]{3mm}{\multirow{10}{*}{\rotatebox[origin=c]{90}{Car}}} &   MUTR3D R50 \cite{zhang2022mutr3d} (CVPRW2022)        &  0.221 & 0.562 & 1329 & 5057 & 18 & 0.086  & 3.836  & 6.897  & 0.449 & 0.257	&	2.183&	3.506&	0.174 \\

     &  MUTR3D R101 \cite{zhang2022mutr3d} (CVPRW2022)                                                                          & 0.258 & 0.513 & 1002  & 5092 & 8  & 0.102 &  3.351 & 6.084  &  0.434&0.304	&		1.834	&2.992&	\underline{0.146}\\
     
     &  ViP3D Det\&Track \cite{gu2023vip3d} (CVPR2023)                                                                           & 0.189 & 0.583 & 1365 & 5300 & 3 & 0.117  & 2.358  & \underline{4.330} & \underline{0.342} & 0.236		&	1.989&	3.117	&0.150\\
     
     &  UniAD Det\&Track \cite{uniad} (CVPR2023)                                                                                 & 0.227 & 0.438 & \underline{950} & 5391 & 18 & 0.140  & 2.483 & 4.529  & 0.372 & 0.278		&	2.093	&3.399&	0.164\\

       \cmidrule(){2-15}

    &  MegVii \cite{zhu2019class}+AB3DMOT \cite{Weng2020_AB3DMOT} (IROS2020)    & 0.281 & 0.289 & 1239 & 4601 & 73 & 0.144  & 2.289 & 4.337  & 0.368 & 0.282	&		2.099&	3.525	&0.165\\
    
     &  CenterPoint \cite{yin2021center} (CVPR2021)                              & \underline{0.398} & \underline{0.221} & {1377} & \underline{3570} & 4 & \underline{0.163}  &  \underline{2.107} &  4.363 & 0.412 & \underline{0.406}		&	\underline{1.571}	&\underline{2.797}	&0.148\\
     
     &  VoxelNext \cite{chen2023voxelnext} (CVPR2023)                            & {0.376} & 0.241 & 1367 & {3765} &\underline{ 1} & 0.158  & 2.108  &  4.363 & 0.416 & 0.388	&		1.664&	2.928&	0.166\\

     \cmidrule(){2-15}
      & GT position and identity         & 0.987 & 0.000 & 103 & 0 & 0 &   0.375 &  1.874 & 3.935  & 0.349 & 0.756		&	1.211&2.305&	0.115 \\
     
     &  GT position + Tracking model \cite{yin2021center}      & 0.971 & 0.001 & 135 & 0 & 103 & 0.368 & 1.915  & 3.970  & 0.351 &0.737	&		1.324&	2.464&	0.122 \\
     \midrule
     \parbox[t]{3mm}{\multirow{10}{*}{\rotatebox[origin=c]{90}{Bus}}} &   MUTR3D R50 \cite{zhang2022mutr3d} (CVPRW2022)        & 0.160 & 0.961 & 165 & 404 & 7 & 0.038  &  4.060 & 7.141 & 0.505 & 0.173	&		2.490&	3.578	&0.183\\

     &  MUTR3D R101 \cite{zhang2022mutr3d} (CVPRW2022)                                                                          & 0.268 & 0.818 & 110 & 391 & 1 & 0.060  &  3.228 & 5.983  & 0.482 & 0.255		&	2.020	&2.867&	0.144\\
     
     &  ViP3D Det\&Track \cite{gu2023vip3d} (CVPR2023)                                                                           & 0.121 & 1.018 & 197 & 406 & \underline{0} & 0.043  & 2.853  & 5.083  & 0.466 &0.173		&	2.132	&3.007&	0.144 \\
     
     &  UniAD Det\&Track \cite{uniad} (CVPR2023)                                                                                 & 0.108 & 0.689 & 130 & 480 & 2 & 0.048    &  3.000 & 5.525 & 0.505 & 0.206		&	2.233	&3.112&	0.171\\

       \cmidrule(){2-15}

    &  MegVii \cite{zhu2019class}+AB3DMOT \cite{Weng2020_AB3DMOT} (IROS2020)    & 0.328 & 0.585 & \underline{61} & 398 & 2 & 0.109 &  2.331 & 4.224  & 0.428  & 0.338		&	1.926	&2.891&	0.123\\
    
     &  CenterPoint \cite{yin2021center} (CVPR2021)                              & 0.445 & \underline{0.466} & {102} & \underline{278} & {1} &  \underline{0.156}  & \underline{2.026}  & \underline{4.081}  & \underline{0.383} & 0.373	&		1.601&	2.632	&0.134\\
     
     &  VoxelNext \cite{chen2023voxelnext} (CVPR2023)                            & \underline{0.480} & 0.484 & 90 & {266} & {1} &  0.106 &  2.196 & 4.562  & 0.512 &\underline{0.478}&			\underline{1.539}&	\underline{2.465}	&\underline{0.113}\\
     


     \cmidrule(){2-15}
     & GT position and identity        & 0.980 & 0.000 & 14 & 0 & 0 & 0.354   & 1.859  & 4.042 & 0.382 & 0.783		&	1.051	&1.976&	0.097\\
     
     &  GT position + Tracking model \cite{yin2021center}      & 0.949 & 0.000 & 14 & 0 & 21 & 0.294 &  1.939 & 4.086  &  0.400 &0.751	&		1.351	&2.401&	0.116\\



     \midrule
     \parbox[t]{3mm}{\multirow{10}{*}{\rotatebox[origin=c]{90}{Truck}}} &   MUTR3D R50 \cite{zhang2022mutr3d} (CVPRW2022)        & -0.129 & 0.886 & 334 & 1235 & 2 & 0.001 &  5.532 & 9.730  & 0.563 & 0.027		&	2.639	&4.067	&0.221\\

     &  MUTR3D R101 \cite{zhang2022mutr3d} (CVPRW2022)                                                                          & -0.083 & 0.807 & 261 & 1244 & 2 & 0.002  & 5.036  &  8.633 & 0.577 &0.035		&	2.436	&3.811&	0.212\\
     
     &  ViP3D Det\&Track \cite{gu2023vip3d} (CVPR2023)                                                                           & -0.103 & 0.945 & 293 & 1241 & \underline{0} & 0.008  & 2.657  & 4.590  & \underline{0.361} & 0.017		&	2.599	&3.989	&0.225\\
     
     &  UniAD Det\&Track \cite{uniad} (CVPR2023)                                                                                 & \underline{0.048}  & 0.723 & 119 & \underline{1205} & \underline{0} & 0.018  & 2.607  &  4.693 & 0.404 & 0.054	&		2.590	&3.978	&0.222 \\

       \cmidrule(){2-15}

    
    &  MegVii \cite{zhu2019class}+AB3DMOT \cite{Weng2020_AB3DMOT} (IROS2020)    & -0.146 & 0.541 & 357 & {1233} & 4 & 0.013 & 3.017 & 5.278  &  0.482  & 0.060		&	2.787	&4.536	&0.239\\
    
     &  CenterPoint \cite{yin2021center} (CVPR2021)                              & {0.004} & {0.358} & \underline{143} & 1242 & \underline{0}& 0.016& \underline{2.110}  & \underline{4.505}  & 0.455 & 0.076	&		1.841&	3.136	&\underline{0.192}\\
     
     &  VoxelNext \cite{chen2023voxelnext} (CVPR2023)                            & -0.031 & \underline{0.285} & 182 & 1252 & \underline{0} & \underline{0.023}  &  2.287 &  4.657 & 0.442 & \underline{0.085}	&		\underline{1.815}&	\underline{3.131}	&0.213\\

     \cmidrule(){2-15}
     & GT position and identity         & 0.973 & 0.000 & 38 & 0 & 0 &  0.300  & 1.966  & 4.211   & 0.408  & 0.733		&	1.309	&2.554&	0.127\\
     
     &  GT position + Tracking model \cite{yin2021center}       & 0.948 & 0.000 & 31 & 0 & 41 & 0.290  & 2.047  &  4.288 &  0.417 & 0.702		&	1.528	&2.863	&0.146 \\



     \midrule
     \parbox[t]{3mm}{\multirow{10}{*}{\rotatebox[origin=c]{90}{All}}} &   MUTR3D R50 \cite{zhang2022mutr3d} (CVPRW2022)        &0.170 & 0.607 & 1828 & 6696 & 27 & 0.042  &  3.993 & 7.151  & 0.463 & 0.152		&	2.237	&3.554	&0.178 \\

     &  MUTR3D R101 \cite{zhang2022mutr3d} (CVPRW2022)                                                                          & 0.213 & 0.550 & 1373 & 6727 & 11 &0.055 & 3.480  & 6.286  &  0.449 & 0.198		&	1.892	&3.043&	\underline{0.150}\\
     
     &  ViP3D Det\&Track \cite{gu2023vip3d} (CVPR2023)                                                                           & 0.145 & 0.636 & 1855 & 6947 & 3 & 0.056  &  2.416 &  4.404 & \underline{0.353} &0.142	&	2.044	&3.173	&0.155 \\
     
     &  UniAD Det\&Track \cite{uniad} (CVPR2023)                                                                                 & 0.195 & 0.471 & \underline{1199} & 7076 & 20 & 0.069  & 2.530  & 4.613  & 0.384 &0.180		&	2.142	&3.424	&0.169\\

       \cmidrule(){2-15}

    &  MegVii \cite{zhu2019class}+AB3DMOT \cite{Weng2020_AB3DMOT} (IROS2020)    & 0.226 & 0.320 & 1657 & 6232 & 79 & 0.089 & 2.356  & 4.412  & 0.382 & 0.227		&	2.143	&3.561	&0.168\\
    
     &  CenterPoint \cite{yin2021center} (CVPR2021)                              & \underline{0.348} & \underline{0.244} & 1622 & \underline{5090} & {5} &  \underline{0.112} & \underline{2.102}   &  \underline{4.354}&  0.413& 0.285		&	\underline{1.596}&	\underline{2.815}&	0.151\\
     
     &  VoxelNext \cite{chen2023voxelnext} (CVPR2023)                            & 0.328 & 0.263& 1639 & 5283 & \underline{2} & 0.096   & 2.134  & 4.409  &  0.426 & \underline{0.317}	&		1.669	&2.914	&0.166\\
     


     \cmidrule(){2-15}
     & GT position and identity        & 0.985 & 0.000 & 155 & 0 & 0 &  0.343  & 1.885  & 3.979  & 0.359 & 0.757		&	1.213&	2.316	&0.115\\
     
     & GT position + Tracking model \cite{yin2021center}      & 0.967 & 0.001 & 180 & 0 & 165 & 0.317  &  1.934 & 4.020  &  0.363 & 0.730			&1.353	&2.513	&0.125\\
     
     
    \bottomrule
    \end{tabular}
    }
  \label{tab:real_world_results_per_class}
\end{table*}



==> tabs/real_world_map_pred.tex <==
\begin{table*}[ht]
\centering

\tabcolsep=0.11cm
    \caption{Online mapping evaluated on nuScenes validation set. BEV segmentation (IoU).}
    \resizebox{0.9\linewidth}{!}{
    \begin{tabular}{c l c c c c c c c c  c}
    \toprule
     & Method & Lane & Road segm. & Driv. area & Road div. & Lane div. & Stop line & Ped. cross. & Walkway & Mean \\ [0.5ex]

     \midrule  &   
    SimpleBeV \cite{harley2022simple} & 0.546 & 0.690 & 0.672 & 0.324 & 0.430 & 0.281 & 0.325 & 0.401 & 0.458 \\
     &  LaRa \cite{bartoccioni2022lara} & 0.465 & 0.610 & 0.599 & 0.230 & 0.317 & 0.159 & 0.200 & 0.310 & 0.361 \\
    \bottomrule
    \end{tabular}
    }
  \label{tab:real_world_map_pred}
\end{table*}


==> tabs/real_world_map_pred_vector.tex <==
\begin{table*}[ht]
\centering

\tabcolsep=0.11cm
    \caption{Performance of vectorized online mapping MapTR (LiDAR + Camera) \cite{MapTR} on nuScenes.}
    \resizebox{0.7\linewidth}{!}{
    \begin{tabular}{c l c c c }
    \toprule
    Dataset & AP\_ped & AP\_divider & AP\_boundary & mAP \\ [0.5ex]

    \midrule  
    nuScenes Train & 92.0 & 97.4 & 94.7 & 94.7 \\
     \midrule  
    nuScenes Validation &  56.5 & 61.8 & 70.1 & 62.8\\
    \bottomrule
    \end{tabular}
    }
  \label{tab:real_world_map_pred_vector}
\end{table*}


==> tabs/tracking_methods.tex <==
\begin{table*}
\centering
\tabcolsep=0.11cm
    \caption{Summary of considered tracking methods.}
    \resizebox{0.9\linewidth}{!}{
    \begin{tabular}{l l c c l}
    \toprule
     \multicolumn{1}{l}{\textbf{Method}} & Conference & Camera-based & Lidar-based & Type of tracking \\ 
    \midrule
     GT position and identity & --- & --- & --- & Ground-truth tracking \\ 
     GT position + Tracking model \cite{yin2021center} &  --- & --- & --- & Simple tracking \\
     MUTR3D R50 \cite{zhang2022mutr3d} & CVPRW 2022 & \cmark & \xmark & Joint detection and tracking \\ 
     MUTR3D R101 \cite{zhang2022mutr3d} & CVPRW 2022 & \cmark & \xmark & Joint detection and tracking \\ 
     ViP3D Det\&Track \cite{gu2023vip3d} & CVPR 2023 & \cmark & \xmark & Forecasting-aware tracking \\ 
     UniAD Det\&Track \cite{uniad} & CVPR 2023 & \cmark & \xmark & Planning-aware tracking \\
     MegVii \cite{zhu2019class} + AB3DMOT \cite{Weng2020_AB3DMOT} & IROS 2020 & \xmark & \cmark & Separate Detection and Tracking \\
     CenterPoint \cite{yin2021center} & CVPR 2021 & \xmark & \cmark & Joint detection and tracking \\ 
     VoxelNext \cite{chen2023voxelnext} & CVPR 2023 & \xmark & \cmark & Joint detection and tracking \\
    \bottomrule
    \end{tabular}
    }
  \label{tab:tracking_methods}
\end{table*}



==> tabs/training_with_da.tex <==
\begin{table}[h]
\centering
    \caption{\yihongh{Finetuning LaPred with data augmentation. The data augumentation is a mixture (Mix) of FP, FN, IDS and Localization error  (Loc. Error) of three different probabilities: 10\%, 30\% and 50\%. The fine-tuning is conducted on the tracking results on the trainset and test on the validation of nuScenes Prediction.}}
    
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l c c c c c}
    \toprule
    Training input & Testing input & mAP${_f}$  $\uparrow$ & minADE $\downarrow$  & minFDE $\downarrow$  & MR $\downarrow$ \\

     \midrule  
     \multirow{16}{*}{Ground truth} & GT  & 0.760 & 1.237 & 2.344 & 0.118 \\  
       &  VoxelNext                                     &  0.317 & 1.669 & 2.914 & 0.166\\ 
       &  UniAD                                        &0.180 &2.142 &3.424 & 0.169 \\  
       & MUTR3D R101                                      &0.198 & 1.892 & 3.043 & 0.150\\ 
       & {10\% FN} & & & & \\
       & {30\% FN} & & & & \\
       & {50\% FN} & & & & \\
       
       & {10\% FP} & & & & \\
       & {30\% FP} & & & & \\
       & {50\% FP} & & & & \\
       
       & {10\% IDS} & & & & \\
       & {30\% IDS} & & & & \\
       & {50\% IDS} & & & & \\
       
       & {10\% Loc. Error} & & & & \\
       & {30\% Loc. Error} & & & & \\
       & {50\% Loc. Error} & & & & \\
     \midrule   

       \multirow{3}{*}{10\% Mix} &  VoxelNext                                     & -0.007	&+0.147	&+0.053&	-0.002\\ 
       &  UniAD                                        &+0.013	&-0.041	&-0.158	&-0.015 \\  
       & MUTR3D R101                                     &+0.015	&-0.016&	-0.154	&-0.006\\ 

       10\% FN & 10\% FN & & & & \\
       10\% FP & 10\% FP & & & & \\
       10\% IDS & 10\% IDS & & & & \\
       10\% Loc. Error & 10\% Loc. Error & & & & \\

    \midrule   
      
      \multirow{3}{*}{30\% Mix} &  VoxelNext                                    & -0.014	&+0.293	&+0.207	&+0.014\\ 
       &  UniAD                                        &+0.005	&-0.117	&-0.234&	-0.006\\  
       & MUTR3D R101                                      &+0.007	&+0.067	&-0.002	&+0.014\\
       30\% FN & 30\% FN & & & & \\
       30\% FP & 30\% FP & & & & \\
       30\% IDS & 30\% IDS & & & & \\
       30\% Loc. Error & 30\% Loc. Error & & & & \\

    \midrule   
       \multirow{3}{*}{50\% Mix} &  VoxelNext            &-0.019	&+0.462	&+0.368	&+0.023\\ 
       &  UniAD                                        &-0.007&	+0.093	&+0.030	&+0.019 \\  
       & MUTR3D R101                                    & -0.013&	+0.236	&+0.221	&+0.036\\
       50\% FN & 50\% FN & & & & \\
       50\% FP & 50\% FP & & & & \\
       50\% IDS & 50\% IDS & & & & \\
       50\% Loc. Error & 50\% Loc. Error & & & & \\

     \midrule   
     \xyhh{100\% Loc. Errors} & \xyhh{100\% Loc. Errors} & 0.619	&2.005	&3.201	&0.189\\
    \bottomrule
    \end{tabular}
    }
  \label{tab:train_da}
\end{table}


==> tabs/visu.tex <==
\begin{figure*}[h]
\centering
\begin{subfigure}{0.24\linewidth}
\includegraphics[trim={0cm 1.8cm 0 2.0cm},clip, width=\linewidth]{figs/visu/FN_crop.png} 
    \vspace{-0.6cm} 
  \caption{FN\vspace{-0.2cm}}
\end{subfigure}
\centering
\begin{subfigure}{0.24\linewidth} 
\includegraphics[trim={0cm 1.8cm 0 2.0cm},clip, width=\linewidth]{figs/visu/FP_crop.png}
    \vspace{-0.6cm} 
  \caption{FP\vspace{-0.2cm}}
\end{subfigure}
\centering
\begin{subfigure}{0.24\linewidth}
\includegraphics[trim={0cm 1.8cm 0 2.0cm},clip, width=\linewidth]{figs/visu/FPFN_crop.png}
    \vspace{-0.6cm} 
  \caption{Localization error\vspace{-0.2cm}}
\end{subfigure}
\centering
\begin{subfigure}{0.24\linewidth}
\includegraphics[trim={0cm 1.8cm 0 2.0cm},clip, width=\linewidth]{figs/visu/IDSW_crop.png}
    \vspace{-0.6cm} 
  \caption{IDS\vspace{-0.2cm}}
\end{subfigure}
\caption{(a) Lost past trajectory causes imprecise forecasting. (b) False positives affect the predicted trajectory. (c) Imprecise past trajectory causes impactful forecasting errors. (d) Identity switching modifies the past trajectory thus creating a different forecasting outcome. (pink) Past trajectory and future forecasts \cite{yuan2021agentformer} with perception inputs \cite{Weng2020_AB3DMOT, zhu2019class}; (orange) future forecasts with curated past inputs; (red) ego car; (green) curated agents and trajectories; (blue) drivable area; (cyan) road lines; (magenta) lane boundaries.}
\label{fig:visu}
\vspace{-6mm}
\end{figure*}

